Variational formulation and monolithic solution of computational homogenization methods

In this contribution, we derive a consistent variational formulation for computational homogenization methods and show that traditional FE2 and IGA2 approaches are special discretization and solution techniques of this most general framework. This allows us to enhance dramatically the numerical analysis as well as the solution of the arising algebraic system. In particular, we expand the dimension of the continuous system, discretize the higher dimensional problem consistently and apply afterwards a discrete null-space matrix to remove the additional dimensions. A benchmark problem, for which we can obtain an analytical solution, demonstrates the superiority of the chosen approach aiming to reduce the immense computational costs of traditional FE2 and IGA2 formulations to a fraction of the original requirements. Finally, we demonstrate a further reduction of the computational costs for the solution of general non-linear problems.

==> sections/basics.tex <==
\section{Governing equations}\label{sec:basics}
We start with a short summary of the governing equations. 
%%%%
%%%%
\subsection{Macro-continuum}
Consider a Lipschitz bounded continuum body in its reference configuration \(\mathcal{B}_{0}\subset\mathbb{R}^{n}\) with \(n\in \{2,3\}\), undergoing a motion characterized by a time-dependent deformation mapping $\vec{\varphi}:\mathcal{B}_{0} \times \mathcal{T}\rightarrow \mathbb{R}^d$, 
$(\vec{X},t)\mapsto\vec{x} = \vec{\varphi}(\vec{X},t)$, which maps at time $t\in \mathcal{T} = [0,\,T]$ material points $\vec{X} \in \mathcal{B}_{0}$ of the reference configuration $\mathcal{B}_{0}$ onto points $\vec{x} \in \mathcal{B}_{t}$ of the current configuration $\mathcal{B}_t = \vec{\varphi}(\mathcal{B}_{0},t)$. The material deformation gradient is defined by $\vec{F}:\mathcal{B}_0\times [0,\,T] \rightarrow\mathbb{R}^{n\times n}$, $\vec{F} = \nablaq{\vec{X}}(\vec{x})$, which maps infinitesimal vectors $\d\vec{X}$ at the material point $\vec{X}$ to the infinitesimal vector $\d \vec{x}$ at $\vec{x}$ in the deformed configuration. An infinitesimal area element, oriented at the material point $\vec{X}$ with the outward, reference normal vector $\vec{N}$ can be defined by two linearly independent vectors via $\d\vec{X}^{(1)}\times \d\vec{X}^{(2)} = \vec{N}\d A$. The well-known Nanson formula reads $\vec{n}\d a = \op{cof}(\vec{F})\vec{N}\d A$,  where $\op{cof}(\vec{F}) = \vec{H}$ is the co-factor,  given by 
\begin{equation}
\vec{H} := \frac{1}{2}(\vec{F}\dcross\vec{F}).
\end{equation}
Here, we apply the cross product of two second-order tensors $\vec{A}$ and $\vec{B}$ with $[\vec{A}\dcross\vec{B}]_{iJ} = \epsilon_{ijk}\epsilon_{JMN}[\vec{A}]_{jM}[\vec{B}]_{kN}$, using the third-order Levi-Civita permutation symbol $\epsilon_{ijk}$. The infinitesimal volume element $\d V$ in the material configuration is related to the deformed counterpart via the Jacobian $J \!:=\!\op{det}[\vec{F}]>0$, where the determinant is defined by
\begin{equation}
\op{det}(\vec{F}) := \frac{1}{6}\vec{F}:(\vec{F}\dcross\vec{F}).
\end{equation}
A graphical representation of the different kinematical values is given in Fig.\ \ref{fig:kin}, see \cite{BETSCH2018660} for further details.

\begin{figure}[htb]
\begin{center} 
\includegraphics[width=0.7\textwidth]{pictures/configuration.eps} 
\caption{Graphical representation kinematical values $\vec{\varphi}$, $\vec{F}$, $\vec{H}$ and $J$, taken from \cite{BETSCH2018660}.}\label{fig:kin}
\end{center}
\end{figure}

Introducing the space of virtual or admissible test functions for the deformation 
\begin{equation}
\mathcal{V}^{\delta\varphi} = \{\delta\vec{\varphi}\in {H}^1(\mathcal{B}_0)\,|\,\delta\vec{\varphi}=\vec{0}\,\text{on}\,\Gamma^{\varphi}\},
\end{equation}
where $\Gamma^{\varphi}\in\partial\mathcal{B}_0$ refers to the Dirichlet boundary,  the internal virtual work  reads
\begin{equation}\label{eq:internal}
\delta\Pi^{\mathrm{int},\varphi} = \int\limits_{\mathcal{B}_0}\vec{P}:\nablaq{\vec{X}}(\delta\vec{\varphi})\,\d V,
\end{equation}
where $\vec{P}$ denotes the first Piola-Kirchhoff stress tensor.  For localization, we apply integration by parts and equilibrate the resulting terms with external contributions
\begin{equation}\label{eq:extern}
\begin{aligned}
\int\limits_{\mathcal{B}_0}\delta\vec{\varphi}\cdot\left[\nablaq{\vec{X}}\cdot\vec{P}^T + \vec{B}\right]\d V &= 0,\\
\int\limits_{\Gamma^\sigma}\delta\vec{\varphi}\cdot\left[\vec{PN} - \vec{T} \right]\d A &= 0,\\
\int\limits_{\Gamma^\varphi}\delta\vec{\varphi}\cdot\left[\vec{\varphi} - \bar{\vec{\varphi}}\right] \d A &= 0,
\end{aligned}
\end{equation}
where $\vec{B}$ is a body load and $\vec{T}$ the Neumann surface load on $\Gamma^\sigma\in \partial\mathcal{B}_0$, assuming that  
$\Gamma^\varphi\cap\Gamma^\sigma = \emptyset$ and $\bar{\Gamma}^\varphi\cup\bar{\Gamma}^\sigma = \partial\mathcal{B}_0$. 

Without prejudice to the generality of the chosen approach, we restrict us here on elastic materials, noting that ductile and general inelastic models can be applied as well. To describe elastic materials in the large strain regime, a well accepted mathematical requirement, the concept of polyconvexity, must be satisfied by the strain energy density function, see \cite{bonet2015a} for details. In particular, we require the strain energy density function $\Psi$ to be a convex multi-valued and inhomogeneous function given by
\begin{equation}\label{eq:constitutive}
\Psi := \Psi(\vec{F}) = \bar{\Psi}(\vec{F},\vec{H},J,\vec{X}),
\end{equation}
where $\bar{\Psi}$ is convex with respect to the 19 values of $\vec{F}$, $\vec{H}$ and $J$. For isotropic materials such as a compressible Moonley-Rivlin material we can assume the constitutive relation to take the form
\begin{equation}\label{eq:MR}
\bar{\Psi}_{MR} := \alpha(\vec{X})\vec{F}:\vec{F} + \beta(\vec{X})\vec{H}:\vec{H} + f(J,\vec{X}), 
\end{equation}
where $\alpha$ and $\beta$ are positive material parameters locally defined at $\vec{X}$ and $f$ is a convex function of $J$ and $\vec{X}$.  The first Piola-Kirchhoff stress tensor follows immediately from
\begin{equation}
\vec{P} := \frac{\partial \Psi}{\partial\vec{F}} = \frac{\partial \bar{\Psi}}{\partial\vec{F}} +  \frac{\partial\bar{\Psi}}{\partial\vec{H}}\dcross\vec{F} + \frac{\partial\bar{\Psi}}{\partial J}\vec{H}.
\end{equation}
With regard to \eqref{eq:extern},  we obtain for the virtual work of the internal and external contributions
\begin{equation}\label{eq:weakMech}
G^{\vec{\varphi}} := \int\limits_{\mathcal{B}_0}\vec{P}:\nablaq{\vec{X}}(\delta\vec{\varphi})\,\d V - \int\limits_{\mathcal{B}_0}\delta\vec{\varphi}\cdot\vec{B}\, \d V -
\int\limits_{\Gamma^\sigma} \delta\vec{\varphi}\cdot\vec{T}\, \d A,
\end{equation} 
to be solved until $G^{\vec{\varphi}} = 0$. 

For later consideration of microstructure information, we introduce internal variables $\tilde{\vec{\omega}}$, such that the strain energy is defined by $\Psi:=\Psi(\vec{F},\vec{H},J,\tilde{\vec{\omega}},\vec{X})$. Therefore, we obtain the additional equation
\begin{equation}\label{eq:internalBalance}
G^{\tilde{\vec{\omega}}} := \int\limits_{\mathcal{B}_0}\frac{\partial\Psi}{\partial\tilde{\vec{\omega}}}\cdot\delta\tilde{\vec{\omega}}\d V,
\end{equation}
to be solved until $G^{\tilde{\vec{\omega}}} = 0$. The exact definition of the internal variables will be given in the next Section.
\begin{remark}
As we will show subsequently for the specific case of FE$^2$ and IGA$^2$ methods, internal variables are often linked to the rest of the system via a set of non-linear equations. Usually, an internal Newton-Raphson iteration is applied, along with a consistent linearization of the global Newton-Raphson iteration. The novel solution method proposed here can be applied most generally for this type of problems. 
\end{remark}
%\begin{remark}
%The considered singlescale continuum theory based on infinitesimal kinematical values $\vec{F}$, $\vec{H}$ and $J$ resolves every possible finite dimensional microstructure,  where the strain energy density function $\Psi := \Psi(\vec{F},\vec{X})$ depends on the actual position in $\mathcal{B}_0$.  As a result,  finite dimensional microcontinua on a different scale to resolve local microstructures cannot exist per definition within an infinitesimal continuum formulation.  As we aim at numerical homogenization procedures of real-world finite dimensional microcontinua, we introduce first the discretization of the singlescale continuum and consider afterwards the solution of microstructures which are not resolved any more.
%\end{remark}
%%%%
%%%%
\subsection{Micro-continuum}
To account for the influence of the underlying microstructure on the material behaviour, we assign a representative 
elementary volume (RVE) $\RVE=\RVE(\vec{X})$ to each point $\vec{X}\in\mathcal{B}_0$, on which we introduce a 
deformation map $\tilde{\vec{\varphi}}:\Omega_{0} \times \mathcal{T}\rightarrow \mathbb{R}^d$ and the quantities derived 
from it analogue to the macro continuum%
%
\footnote{In order to distinguish between corresponding macro- and micro-entities, all quantities of the micro-continuum 
will be marked with a superimposed tilde.}.
% 
The material of $\RVE$ is described by a convex strain energy density function $\tilde{\Psi}$, and we assume that 
the macroscopic and microscopic gradients $\vec{F}$, $\tilde{\vec{F}}$ as well as the elastic potentials $\Psi$, $\tilde{\Psi}$ 
are related via the volume averages
\begin{equation}\label{eq:homogenization}
\vec{F}=\frac{1}{|\RVE|}\int\limits_{\RVE}\tilde{\vec{F}}\,\d \tilde{V}\quad\text{and}\quad
\Psi=\frac{1}{|\RVE|}\int\limits_{\RVE}\tilde{\Psi}\,\d \tilde{V},
\end{equation}
where $|\RVE|$ is the volume of $\RVE$. In addition, we assume a static equilibrium state of the 
micro-continuum governed by the field equation
\begin{equation}\label{eq:microStat}
\nablaq{\tilde{\vec{X}}}\cdot \tilde{\vec{P}} = \vec{0},\quad \text{in }\RVE
\end{equation} 
and the deformation $\tilde{\vec{\varphi}}$ to be linked to the underlying point $\vec{X}\in\mathcal{B}_0$ 
in the macro-continuum via a first order Taylor expansion%
%
\footnote{As shown in \cite{hesch2022}, we obtain a higher-order Taylor expansion in the context of higher-order problems.} 
%
\begin{equation}\label{eq:microdefo}
\tilde{\vec{\varphi}}(\tilde{\vec{X}}) = \vec{F}(\vec{X})\tilde{\vec{X}} + \tilde{\vec{w}}(\tilde{\vec{X}}),\quad 
\tilde{\vec{X}}\in\RVE,
\end{equation} 
such that the micro deformation consists of a homogeneous part $\vec{F}(\vec{X})\tilde{\vec{X}}$ and a non-homogeneous 
field $\tilde{\vec{w}}\colon\RVE\to\mathbb{R}^n$ referred to as microscopic fluctuations. According to 
Eq.\ \eqref{eq:microdefo}, we obtain 
\begin{equation}\label{eq:microGrad}
\tilde{\vec{F}} = \nablaq{\tilde{\vec{X}}}(\tilde{\vec{\varphi}}) = 
\vec{F}(\vec{X}) + \vec{F}',\quad \vec{F}':=\nablaq{\tilde{\vec{X}}}(\tilde{\vec{w}}),
\end{equation}
so that for homogeneous materials with zero fluctuations, $\vec{F}(\vec{X})$ is recovered for the micro deformation gradient. 
In addition, insertion of \eqref{eq:microGrad} into \eqref{eq:homogenization}$_1$ yields the constraint
\begin{equation}\label{eq:fluctuCon}
\vec{F}=\vec{F}+\frac{1}{|\RVE|}\int_{\RVE} \nablaq{\tilde{\vec{X}}}(\tilde{\vec{w}})\,\d \tilde{V}
\;\Longleftrightarrow\;
\int\limits_{\RVE}\nablaq{\tilde{\vec{X}}}(\tilde{\vec{w}})\,\d \tilde{V} = \vec{0}
\end{equation} 
for the superimposed deformation field $\tilde{\vec{w}}$ and 
with Eq.\ \eqref{eq:homogenization}$_2$ we obtain a relationship between macro- and micro-stress as follows  
\begin{equation}
\vec{P}=\frac{\partial\Psi}{\partial\vec{F}} = 
\frac{1}{|\RVE|}\int\limits_{\RVE}\frac{\partial\tilde{\Psi}}{\partial \vec{F}}\,\d \tilde{V} =
\frac{1}{|\RVE|}\int\limits_{\RVE}\frac{\partial\tilde{\Psi}}{\partial \tilde{\vec{F}}}
\frac{\partial\tilde{\vec{F}}}{\partial \vec{F}}\,\d \tilde{V} = 
\frac{1}{|\RVE|}\int\limits_{\RVE}\tilde{\vec{P}}\,\d \tilde{V},
\end{equation}
where we have utilised in the last equation that according to \eqref{eq:microGrad}, 
$\partial\tilde{\vec{F}}/\partial\vec{F}$ is the identity. 
Applying Gauss divergence theorem, the constraint \eqref{eq:fluctuCon} can be alternatively 
expressed as 
\begin{equation}\label{eq:boundaryA}
\int\limits_{\partial\RVE}\tilde{\vec{w}}\otimes\tilde{\vec{N}}\,\d \tilde{A} = \vec{0},
\end{equation}
showing that \eqref{eq:fluctuCon} is satisfied by the alternative conditions
\begin{equation}\label{eq:Con}
\text(i)\;   \tilde{\vec{w}}=\vec{0}\quad\text{in }\RVE, \qquad
\text(ii)\;  \tilde{\vec{w}}=\vec{0}\quad\text{on }\partial\RVE, \qquad 
\text(iii)\; \tilde{\vec{w}}^+=\vec{w}^-\quad\text{on }\partial\RVE,
\end{equation} 
cf.\ Miehe~\cite{miehe_computational_1999-1}. The trivial condition $\text{(i)}$ enforces a homogeneous deformation of the entire domain and is usually 
denoted as Taylor assumption, condition $\text{(ii)}$ demands homogeneous deformations on the boundary and $\text{(iii)}$ 
addresses periodic boundary conditions. 
%
\begin{remark}
Each of the three conditions \eqref{eq:Con}, together with \eqref{eq:microStat}, ensures that
the macro-homogeneity condition
\begin{equation}\label{eq:hillA}
\frac{1}{|\RVE|}\int\limits_{\RVE}\tilde{\vec{P}}:\delta\tilde{\vec{F}}\,\d \tilde{V} = 
\vec{P}:\delta\vec{F},
\end{equation} 
also known as Hill-Mandel criterion, is fulfilled. The virtual work applied in a specific 
point $\vec{X}\in\mathcal{B}_0$ to the system thus corresponds to the volumetric average of the 
virtual work in the associated RVE $\RVE(\vec{X})$.
\end{remark}
%Integration by parts of the integral on the left hand side of the last equation yields
%\begin{equation}\label{eq:intbypartsA}
%\int\limits_{\RVE}\tilde{\vec{P}}:\nablaq{\tilde{\vec{X}}}(\delta\tilde{\vec{\varphi}})\,\d \tilde{V} =
%\int\limits_{\partial\RVE}\tilde{\vec{P}}\tilde{\vec{N}}\cdot\delta\tilde{\vec{\varphi}}\,\d \tilde{A} -
%\int\limits_{\RVE}(\nablaq{\tilde{\vec{X}}}\cdot\tilde{\vec{P}})\cdot\delta\tilde{\vec{\varphi}}\,\d \tilde{V}.
%\end{equation}
%Assuming the absence of gravitational forces and Neumann boundary conditions within the micro-continuum, we 
%insert \eqref{eq:microdefo} in \eqref{eq:intbypartsA} and obtain
%\begin{equation}\label{eq:localMicroA}
%\int\limits_{\RVE}\tilde{\vec{P}}:\delta\tilde{\vec{F}}\,\d \tilde{V} =
%\int\limits_{\partial\RVE}\tilde{\vec{P}}\tilde{\vec{N}}\otimes\tilde{\vec{X}}\,\d \tilde{A}:
%\delta\vec{F},
%\end{equation}
%noting that the macroscopic stresses do not depend on the fluctuations by construction regarding \eqref{eq:boundaryA}, i.e.
%\begin{equation}\label{eq:bounWA}
%\int\limits_{\partial\RVE}\tilde{\vec{P}}\tilde{\vec{N}}\cdot\delta\tilde{\vec{w}}\,\d \tilde{A} = 0.
%\end{equation}
%%%%
%%%%
\subsection{Variational formulation}
Taking into account the relations \eqref{eq:homogenization}$_2$ and \eqref{eq:microGrad} between the elastic potentials $\Psi$, $\tilde{\Psi}$ and 
the gradients $\vec{F}$, $\tilde{\vec{F}}$, $\vec{F}'$, the macro-deformation and micro-fluctuation are determined as minimizer of 
the systems total energy, i.e.\ $\vec{\varphi}$ and $\tilde{\vec{w}}$ have to fulfil the condition
\begin{equation}\label{eq:min1}
(\vec{\varphi},\tilde{\vec{w}})=\arginf_{(\vec{u},\vec{v})\in\mathcal{S}^{\vec{\varphi}}\times 
\mathcal{S}^{\tilde{\vec{w}}}}\left\{\Pi^\mathrm{int}(\vec{u},\vec{v})-\Pi^\mathrm{ext}(\vec{u})\right\}
\end{equation}
where $\mathcal{V}^{\vec{\varphi}}$ and $\mathcal{V}^{\tilde{\vec{w}}}$ are suitable spaces of admissible solutions 
and the internal and external energy contributions are given by
\begin{equation}
\Pi^\mathrm{int}(\vec{u},\vec{v}) = \int\limits_{\mathcal{B}_0}\frac{1}{|\RVE|}\int\limits_{\RVE} 
\tilde{\Psi}[\tilde{\vec{F}}(\vec{F}[\vec{u}],\vec{F}'[\vec{v}])]\,\d\tilde{V}\,\d V,\quad
\Pi^\mathrm{ext}(\vec{u}) = \int\limits_{\mathcal{B}_0}\vec{B}\cdot\vec{u}\,\d V+
\int\limits_{\Gamma^{\sigma}} \vec{T}\cdot\vec{u}\, \d A.
\end{equation}
It should be noted that, according to the assumptions in the previous section, no external contributions 
from the micro-continuum need to be taken into account. Furthermore, it is assumed here that both the body  
load and the Neumann surface load are independent of the deformation. Introducing the spaces of virtual deformations 
and fluctuations
\begin{equation}
...
\end{equation}
standard variational calculus finally yields the variational problem: find $(\vec{\varphi},\tilde{\vec{w}})\in 
\mathcal{V}^{\vec{\varphi}}\times\mathcal{V}^{\tilde{\vec{w}}}$, so that   
for all $(\delta\vec{\varphi},\delta\tilde{\vec{w}})\in\mathcal{V}^{\delta\vec{\varphi}}\times 
\mathcal{V}^{\delta\tilde{\vec{w}}}$
\begin{equation}\label{eq:varProb}
\begin{aligned}
&\int\limits_{\mathcal{B}_0}\vec{P}:\nablaq{\vec{X}}(\delta\vec{\varphi})-\vec{B}\cdot\delta\vec{\varphi}\,\d V-
\int\limits_{\Gamma^{\sigma}} \vec{T}\cdot \delta\vec{\varphi}\, \d A +
\int\limits_{\mathcal{B}_0} \frac{1}{|\RVE|}\int\limits_{\RVE} \tilde{\vec{P}}:\nablaq{\tilde{\vec{X}}}
(\delta\tilde{\vec{w}})\,\d \tilde{V}\,\d V = 0
\end{aligned}
\end{equation}
\textcolor{red}{Macht so keinen Sinn! Jedem $\vec{X}\in\mathcal{B}_0$ wird ein RVE $\RVE(\vec{X})$ und damit 
eine Mikrofluktuation $\tilde{\vec{w}}_{\vec{X}}$ zugewiesen. D.h.\ wir haben $\infty$-viele $\tilde{\vec{w}}$ 
(ueberabzaehlbar)! Formulierung von \eqref{eq:min1} passt schon nicht!}







   



